Exchange-of-Thought: Enhancing Large Language Model Capabilities through Cross-Model Communication

Large Language Models (LLMs) have recently made significant strides in complex reasoning tasks through the Chain-of-Thought technique. Despite this progress, their reasoning is often constrained by their intrinsic understanding, lacking external insights. To address this, we propose Exchange-of-Thought (EoT), a novel framework that enables cross-model communication during problem-solving. Drawing inspiration from network topology, EoT integrates four unique communication paradigms: Memory, Report, Relay, and Debate. This paper delves into the communication dynamics and volume associated with each paradigm. To counterbalance the risks of incorrect reasoning chains, we implement a robust confidence evaluation mechanism within these communications. Our experiments across diverse complex reasoning tasks demonstrate that EoT significantly surpasses established baselines, underscoring the value of external insights in enhancing LLM performance. Furthermore, we show that EoT achieves these superior results in a cost-effective manner, marking a promising advancement for efficient and collaborative AI problem-solving.

==> appendices/appendices-tables/case-init.tex <==
\begin{table}[ht]
\begin{tabular}{p{13cm}}

\toprule
\midrule
\textbf{Q}: Carla is downloading a 200 GB file. Normally she can download 2 GB/minute, but 40\% of the way through the download, Windows forces a restart to install updates, which takes 20 minutes. Then Carla has to restart the download from the beginning. How load does it take to download the file? \\
\midrule
\begin{minipage}[b]{0.16\columnwidth}
    \centering
    \raisebox{-.1in}{\includegraphics[width=\linewidth]{appendices/icons/Kitty.png}}
\end{minipage}
\textbf{Kitty's Solution}: Carla was able to download for 40\% of the time before the restart. 40\% of 200 GB is 80 GB. Since she can download 2 GB/minute, it would take her 80/2 = 40 minutes to download 80 GB. After the forced restart, she has to restart the download from the beginning, so she would need another 200/2 = 100 minutes to complete the download. Plus the 20 minutes for the restart, the total time would be 40 + 100 + 20 = 160 minutes. So the answer is 160 minutes.
\\
\midrule
% \vspace{-1mm}
\begin{minipage}[b]{0.16\columnwidth}
    \centering
    \raisebox{-.1in}{\includegraphics[width=\linewidth]{appendices/icons/Ben.png}}
\end{minipage}
\textbf{Ben's Solution}: Carla needs to download a 200 GB file. Normally, she can download 2 GB/minute, which means it would take her 200 / 2 = 100 minutes to download the file. However, 40\% of the way through the download, Windows forces a restart for 20 minutes, which means Carla has downloaded 200 * 0.4 = 80 GB before the restart. After the restart, she needs to start the download again from the beginning, so the total time it takes her would be 100 + (200 / 2) = 200 minutes. Therefore, it takes Carla 200 minutes to download the file. So the answer is 200 minutes.
\\
\midrule
\begin{minipage}[b]{0.16\columnwidth}
    \centering
    \raisebox{-.1in}{\includegraphics[width=\linewidth]{appendices/icons/Peter.png}}
\end{minipage}
\textbf{Peter's Solution}: Carla can download 2 GB in 1 minute, so to download 200 GB, it will take her 200/2 = 100 minutes if she didn't have to restart. However, she was 40\% of the way through the download when Windows forced the restart, so she had already downloaded 0.4 x 200 = 80 GB. The restart took 20 minutes, so she lost 20 x 2 = 40 GB of progress. After the restart, she had to start again from 0 GB. So in total, she had to download 200 - 80 - 40 = 80 GB. At her regular download speed of 2 GB/minute, it will take her 80/2 = 40 minutes to download the remaining 80 GB. Adding the 20 minutes of the Windows update, the total time it takes Carla to download the file is 20 + 40 = 60 minutes. So the answer is 60 minutes.
\\
\midrule
\bottomrule

\caption{Solutions provided by each character before the discussion begins.} 
\label{table:case-init}
\end{tabular}
\end{table}


==> appendices/sections/baselines.tex <==
\section{Baselines}
\label{appendix:app-baselines}
